Multimodal Motion Conditioned Diffusion Model for Skeleton-based Video Anomaly Detection

Anomalies are rare and anomaly detection is often therefore framed as One-Class Classification (OCC), i.e. trained solely on normalcy. Leading OCC techniques constrain the latent representations of normal motions to limited volumes and detect as abnormal anything outside, which accounts satisfactorily for the openset'ness of anomalies. But normalcy shares the same openset'ness property since humans can perform the same action in several ways, which the leading techniques neglect. We propose a novel generative model for video anomaly detection (VAD), which assumes that both normality and abnormality are multimodal. We consider skeletal representations and leverage state-of-the-art diffusion probabilistic models to generate multimodal future human poses. We contribute a novel conditioning on the past motion of people and exploit the improved mode coverage capabilities of diffusion processes to generate different-but-plausible future motions. Upon the statistical aggregation of future modes, an anomaly is detected when the generated set of motions is not pertinent to the actual future. We validate our model on 4 established benchmarks: UBnormal, HR-UBnormal, HR-STC, and HR-Avenue, with extensive experiments surpassing state-of-the-art results.

==> Tables/aggregator.tex <==
\begin{table}[ht]
\centering{%
\begin{tabular}{lcc}
\hline

  & \textbf{UBnormal} & \textbf{HR-UBnormal}\\ 
\hline
\hline
 Unique generation    &  65.09 &   65.13    \\
 \hline
 Mean of the Generations  & 65.23 &  65.29     \\
 Best Generation   &  65.22 &  65.31     \\
 Worst Generation  & \textbf{\ubnres} &  \textbf{\hrubnres}      \\

\hline
\end{tabular}}
\caption{Ablation study on the type of aggregator chosen to handle multiple generations \AF{this will be included in the discussion section. }
}

\label{tab:aggregator}
\end{table}


==> Tables/res_ubnormal.tex <==
\begin{table}[t]

\centering{

\caption{
\AF{la table di MoCoDAD Vs. Supervised and Weakly supervised è stata spostata nel supplementary}}
\label{tab:ubnormal}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{lcc} 
\toprule
& \multicolumn{1}{c}{\textbf{UBnormal}}  & \multicolumn{1}{c}{\textbf{HR-UBnormal}} \\ 

% \cline{3-4}
% % \cline{6-6}
% \multicolumn{1}{l}{}                                &      & Test  & Test                       \\ 
\midrule
% & \citen{Sultani et al. (CVPR '18)} \cite{sultani18} (pre-trained)                                                       &                     61.1       & 49.5           &     -             \\ 
% \rowcolor{Gray}
\textcolor{gray}{\citen{Sultani} \cite{sultani18} $\dag$}                                                      &                     \textcolor{gray}{50.3}           &     \textcolor{gray}{-}             \\ 
% \rowcolor{Gray} 
\textcolor{gray}{AED-SSMTL  \cite{Georgescu21} $\dag$}                                                                        &  \textcolor{gray}{61.3}            &     \textcolor{gray}{-}     \\ 
% \textit{S}& \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/4$ sample rate. fine-tuned)                  & 78.5       & 61.9             &     -         \\
% & \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/8$ sample rate. fine-tuned)                  & 83.4       & 64.1             &     -         \\
% \rowcolor{Gray}
 \textcolor{gray}{TimeSformer \cite{bertasius21} $\dag$}                   &  \textcolor{gray}{68.5}             &     \textcolor{gray}{-}         \\
% \rowcolor{Gray}
% \textit{\multirow{-4}{*}{\textcolor{gray}{S}}} & \textcolor{gray}{\citen{Barbalau} (CVIU '23)~\cite{barbalau23}} & \textcolor{gray}{62.1} & \textcolor{gray}{-} \\
% \rowcolor{Gray}
\textcolor{gray}{AED-SSMTL \cite{Georgescu21} $\ddag$}                                       &                            \textcolor{gray}{59.3}       & \textcolor{gray}{-}                 \\
MPED-RNN \cite{morais19} $*$                                                                 &  60.6  & 61.2                     \\ 

GEPC \cite{markovitz20} $*$                                           &      53.4   & 55.2                    \\
SSMTL++ ~\cite{barbalau23} & 62.1 & - \\
COSKAD \cite{flaborea23} $*$ &  65.0         & 65.5          \\
\midrule
\OUR\ $*$ &   \textbf{\ubnres} &  \textbf{\hrubnres} \\
\bottomrule
\end{tabular}
}
}
\vspace*{-2mm}

\end{table}

% \begin{table}[t]
% \centering{

% \caption{The table displays AUC values for UBnormal and HR-UBnormal datasets, divided by method framework: gray-colored methods are Supervised or Weakly supervised~($^\dag$), and we include them for reference (cf. Sec.~\ref{sec:experiments}), while black-colored are OCC (One-Class-Classification) methods, comparable with ours. Models for detecting anomalies using skeletons are denoted by the symbol *.}
% \label{tab:ubnormal}
% \begin{tabular}{lcc} 
% \toprule
% & \multicolumn{1}{c}{\textbf{UBnormal}}  & \multicolumn{1}{c}{\textbf{HR-UBnormal}} \\ 

% % \cline{3-4}
% % % \cline{6-6}
% % \multicolumn{1}{l}{}                                &      & Test  & Test                       \\ 
% \midrule
% \midrule
% % & \citen{Sultani et al. (CVPR '18)} \cite{sultani18} (pre-trained)                                                       &                     61.1       & 49.5           &     -             \\ 
% % \rowcolor{Gray}
% \textcolor{gray}{SULTANI \cite{sultani18}}                                                      &                     \textcolor{gray}{50.3}           &     \textcolor{gray}{-}             \\ 
% % \rowcolor{Gray} 
% \textcolor{gray}{AED-SSMTL  \cite{Georgescu21} }                                                                        &  \textcolor{gray}{61.3}            &     \textcolor{gray}{-}     \\ 
% % \textit{S}& \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/4$ sample rate. fine-tuned)                  & 78.5       & 61.9             &     -         \\
% % & \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/8$ sample rate. fine-tuned)                  & 83.4       & 64.1             &     -         \\
% % \rowcolor{Gray}
%  \textcolor{gray}{TimeSformer \cite{bertasius21}}                   &  \textcolor{gray}{68.5}             &     \textcolor{gray}{-}         \\
% % \rowcolor{Gray}
% % \textit{\multirow{-4}{*}{\textcolor{gray}{S}}} & \textcolor{gray}{\citen{Barbalau} (CVIU '23)~\cite{barbalau23}} & \textcolor{gray}{62.1} & \textcolor{gray}{-} \\
% \hline
% % \rowcolor{Gray}
% \textcolor{gray}{AED-SSMTL \cite{Georgescu21} $^\dag$}                                       &                            \textcolor{gray}{59.3}       & \textcolor{gray}{-}                 \\
% \hline
% MPED-RNN \cite{morais19} *                                                                 &  60.6  & 61.2                     \\ 

% GEPC\cite{markovitz20} *                                           &      53.4   & 55.2                    \\
% SSMTL++ ~\cite{barbalau23} *& 62.1 & - \\
% COSKAD \cite{flaborea23} * &  65.0         & 65.5          \\

% \OUR\ * &   \textbf{67.35} &  \textbf{67.37} \\
% \bottomrule
% \end{tabular}
% }

% \end{table}


% \begin{table}[t]
% \centering{

% \caption{The table displays AUC values for UBnormal and HR-UBnormal datasets, divided by method framework: gray-colored methods are Supervised or Weakly supervised~($^\dag$), and we include them for reference (cf. Sec.~\ref{sec:experiments}), while black-colored are OCC (One-Class-Classification) methods, comparable with ours. Models for detecting anomalies using skeletons are denoted by the symbol *.}
% \label{tab:ubnormal}
% \begin{tabular}{lcc} 
% \toprule
% & \multicolumn{1}{c}{\textbf{UBnormal}}  & \multicolumn{1}{c}{\textbf{HR-UBnormal}} \\ 

% % \cline{3-4}
% % % \cline{6-6}
% % \multicolumn{1}{l}{}                                &      & Test  & Test                       \\ 
% \midrule
% \midrule
% % & \citen{Sultani et al. (CVPR '18)} \cite{sultani18} (pre-trained)                                                       &                     61.1       & 49.5           &     -             \\ 
% % \rowcolor{Gray}
% \textcolor{gray}{\citen{Sultani} \cite{sultani18}}                                                      &                     \textcolor{gray}{50.3}           &     \textcolor{gray}{-}             \\ 
% % \rowcolor{Gray} 
% \textcolor{gray}{\citen{Georgescu}  \cite{Georgescu21} }                                                                        &  \textcolor{gray}{61.3}            &     \textcolor{gray}{-}     \\ 
% % \textit{S}& \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/4$ sample rate. fine-tuned)                  & 78.5       & 61.9             &     -         \\
% % & \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/8$ sample rate. fine-tuned)                  & 83.4       & 64.1             &     -         \\
% % \rowcolor{Gray}
%  \textcolor{gray}{\citen{Bertasius} \cite{bertasius21}}                   &  \textcolor{gray}{68.5}             &     \textcolor{gray}{-}         \\
% % \rowcolor{Gray}
% % \textit{\multirow{-4}{*}{\textcolor{gray}{S}}} & \textcolor{gray}{\citen{Barbalau} (CVIU '23)~\cite{barbalau23}} & \textcolor{gray}{62.1} & \textcolor{gray}{-} \\
% \hline
% % \rowcolor{Gray}
% \textcolor{gray}{\citen{Georgescu} \cite{Georgescu21}$^\dag$}                                       &                            \textcolor{gray}{59.3}       & \textcolor{gray}{-}                 \\
% \hline
% \citen{Morais} \cite{morais19} *                                                                 &  60.6  & 61.2                     \\ 

% \citen{Markovitz} \cite{markovitz20} *                                           &      53.4   & 55.2                    \\
% \citen{Barbalau} ~\cite{barbalau23} & 62.1 & - \\
% \citen{Flaborea} \cite{flaborea23} * &  65.0         & 65.5          \\

% Ours * &   \textbf{67.35} &  \textbf{67.37} \\
% \bottomrule
% \end{tabular}
% }

% \end{table}

% \begin{table*}[!ht]
% \centering{

% \caption{The table displays AUC values for UBnormal and HR-UBnormal datasets, divided by method framework: S (Supervised), WS (Weakly-Supervised), and OCC (One-Class-Classification). Models for detecting anomalies using skeletons are denoted by the symbol *. Our results are in bold and should be compared with other OCC methods.}
% \label{tab:ubnormal}

% \begin{tabular}{llcccc} 
% \toprule
% \multicolumn{2}{c}{}                                    &                          \multicolumn{1}{c}{\textbf{UBnormal}}  & \multicolumn{1}{c}{\textbf{HR-UBnormal}} \\ 

% % \cline{3-4}
% % % \cline{6-6}
% % \multicolumn{1}{l}{}                                &      & Test  & Test                       \\ 
% \midrule
% \midrule
% % & \citen{Sultani et al. (CVPR '18)} \cite{sultani18} (pre-trained)                                                       &                     61.1       & 49.5           &     -             \\ 
% % \rowcolor{Gray}
% & \textcolor{gray}{\citen{Sultani} (CVPR '18) \cite{sultani18}}                                                      &                     \textcolor{gray}{50.3}           &     \textcolor{gray}{-}             \\ 
% % \rowcolor{Gray} 
% & \textcolor{gray}{\citen{Georgescu} (TPAMI '21) \cite{Georgescu21} + UBnormal anom.}                                                                       &  \textcolor{gray}{61.3}            &     \textcolor{gray}{-}     \\ 
% % \textit{S}& \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/4$ sample rate. fine-tuned)                  & 78.5       & 61.9             &     -         \\
% % & \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/8$ sample rate. fine-tuned)                  & 83.4       & 64.1             &     -         \\
% % \rowcolor{Gray}
% \textit{\multirow{-3}{*}{\textcolor{gray}{S}}} & \textcolor{gray}{\citen{Bertasius} (ICML '21) \cite{bertasius21}}                   &  \textcolor{gray}{68.5}             &     \textcolor{gray}{-}         \\
% % \rowcolor{Gray}
% % \textit{\multirow{-4}{*}{\textcolor{gray}{S}}} & \textcolor{gray}{\citen{Barbalau} (CVIU '23)~\cite{barbalau23}} & \textcolor{gray}{62.1} & \textcolor{gray}{-} \\
% \hline
% % \rowcolor{Gray}
% \textit{\textcolor{gray}{WS}} & \textcolor{gray}{\citen{Georgescu} (TPAMI '21) \cite{Georgescu21}}                                            &                            \textcolor{gray}{59.3}       & \textcolor{gray}{-}                 \\
% \hline
% &  \citen{Morais} (CVPR '19) \cite{morais19} *                                                                 &  60.6  & 61.2                     \\ 

% &  \citen{Markovitz} (CVPR '20) \cite{markovitz20} *                                           &      53.4   & 55.2                    \\
% & \citen{Barbalau} (CVIU '23)~\cite{barbalau23} & 62.1 & - \\
% &  \citen{Flaborea} (arxiv '23) \cite{flaborea23} * &  65.0         & 65.5          \\

% \textit{\multirow{-5}{*}{OCC}}  & Ours * &   \textbf{67.35} &  \textbf{67.37} \\
% \bottomrule
% \end{tabular}
% }

% \end{table*}






% \begin{table*}[!ht]
% \centering{

% \caption{The table displays AUC values for UBnormal and HR-UBnormal datasets, divided by method framework: S (Supervised), WS (Weakly-Supervised), and OCC (One-Class-Classification). Models for detecting anomalies using skeletons are denoted by the symbol *. Our results are in bold and should be compared with other OCC methods.}
% \label{tab:ubnormal}

% \begin{tabular}{llcccc} 
% \toprule
% \multicolumn{2}{c}{}                                              &                          \multicolumn{1}{c}{\textbf{UBnormal}}  & \multicolumn{1}{c}{\textbf{HR-UBnormal}} \\ 

% % \cline{3-4}
% % % \cline{6-6}
% % \multicolumn{1}{l}{}                                &      & Test  & Test                       \\ 
% \midrule
% \midrule
% % & \citen{Sultani et al. (CVPR '18)} \cite{sultani18} (pre-trained)                                                       &                     61.1       & 49.5           &     -             \\ 
% % \rowcolor{Gray}
% & \textcolor{gray}{\citen{Sultani} (CVPR '18) \cite{sultani18}}                                                      &                     \textcolor{gray}{50.3}           &     \textcolor{gray}{-}             \\ 
% % \rowcolor{Gray} 
% & \textcolor{gray}{\citen{Georgescu} (TPAMI '21) \cite{Georgescu21} + UBnormal anom.}                                                                       &  \textcolor{gray}{61.3}            &     \textcolor{gray}{-}     \\ 
% % \textit{S}& \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/4$ sample rate. fine-tuned)                  & 78.5       & 61.9             &     -         \\
% % & \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/8$ sample rate. fine-tuned)                  & 83.4       & 64.1             &     -         \\
% % \rowcolor{Gray}
% \textit{\multirow{-3}{*}{\textcolor{gray}{S}}} & \textcolor{gray}{\citen{Bertasius} (ICML '21) \cite{bertasius21}}                   &  \textcolor{gray}{68.5}             &     \textcolor{gray}{-}         \\
% % \rowcolor{Gray}
% % \textit{\multirow{-4}{*}{\textcolor{gray}{S}}} & \textcolor{gray}{\citen{Barbalau} (CVIU '23)~\cite{barbalau23}} & \textcolor{gray}{62.1} & \textcolor{gray}{-} \\
% \hline
% % \rowcolor{Gray}
% \textit{\textcolor{gray}{WS}} & \textcolor{gray}{\citen{Georgescu} (TPAMI '21) \cite{Georgescu21}}                                            &                            \textcolor{gray}{59.3}       & \textcolor{gray}{-}                 \\
% \hline
% &  \citen{Morais} (CVPR '19) \cite{morais19} *                                                                 &  60.6  & 61.2                     \\ 

% &  \citen{Markovitz} (CVPR '20) \cite{markovitz20} *                                           &      53.4   & 55.2                    \\
% & \citen{Barbalau} (CVIU '23)~\cite{barbalau23} & 62.1 & - \\
% &  \citen{Flaborea} (arxiv '23) \cite{flaborea23} * &  65.0         & 65.5          \\

% \textit{\multirow{-5}{*}{OCC}}  & Ours * &   \textbf{67.35} &  \textbf{67.37} \\
% \bottomrule
% \end{tabular}
% }

% \end{table*}



% \begin{table*}[!ht]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llcccc} 
% \hline
% \multicolumn{2}{c}{}                                              &                          \multicolumn{2}{c}{\textbf{UBnormal}}  & \multicolumn{1}{c}{\textbf{HR-UBnormal}} \\ 

% \cline{3-5}
% % \cline{6-6}
% \multicolumn{1}{l}{}                                &     &  Validation & Test  & Test                       \\ 
% \hline
% \hline
% % & \citen{Sultani et al. (CVPR '18)} \cite{sultani18} (pre-trained)                                                       &                     61.1       & 49.5           &     -             \\ 
% & \citen{Sultani et al. (CVPR '18)} \cite{sultani18}                                                      &                     51.8       & 50.3           &     -             \\ 

% \textit{\multirow{2}{*}{S}} & \citen{Georgescu et al. (TPAMI '21)} \cite{Georgescu21} + UBnormal anom.                                                                       & 68.2       & 61.3            &     -     \\ 
% % \textit{S}& \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/4$ sample rate. fine-tuned)                  & 78.5       & 61.9             &     -         \\
% % & \citen{Bertasius et al. (ICML '21)} \cite{bertasius21} ($1/8$ sample rate. fine-tuned)                  & 83.4       & 64.1             &     -         \\
% & \citen{Bertasius et al. (ICML '21) } \cite{bertasius21}                   & 86.1       & 68.5             &     -         \\
% & \citen{Barbalau et al. (CVIU '23)}~\cite{barbalau23} & - & 62.1 & - \\
% \hline
% \textit{WS} & \citen{Georgescu et al. (TPAMI '21)} \cite{Georgescu21}                                            &                            58.5       & 59.3       & -                 \\
% \hline
% &  \citen{Morais et al. (CVPR '19)} \cite{morais19} *                                                                 & 61.2          & 60.6  & 61.2                     \\ 

% \textit{\multirow{2}{*}{OCC}} &  \citen{Markovitz et al. (CVPR '20)} \cite{markovitz20} *                                           &     47.0        & 53.4   & 55.2                    \\
% &  \citen{Flaborea et al. (arxiv '23)} \cite{flaborea23} * & 76.4     & 65.0         & 65.5          \\

% \textit{} & Ours * &  \textbf{77.6} &  \textbf{67.1} &  \textbf{66.38} \\
% \hline
% \end{tabular}
% }
% \caption{%Results on the dataset UBnormal and its subset HR-UBnormal, measured in terms of AUC score. The blocks split the table according to the framework each method relies on, where $S$, $WS$, and $OCC$ stand for \textit{Supervised}, \textit{Weakly-Supervised}, and \textit{One-Class-Classification}, respectively. (*) indicates that the model is designed for skeleton-based anomaly detection. We highlight in bold our results, which should be directly compared to the other OCC methods. %We also include in the table some supervised methods to give the reader some context. 
% \TD{need to decide whether to keep or not the validation column}}
% \label{tab:ubnormal}

% \end{table*}


==> Tables/stc_ave.tex <==
\begin{table}[t]
\small
\centering
\caption{\TD{Comparative evaluation on HR-ShangaiTech Campus (HR-STC) and HR-Avenue, in terms of AUC scores.}
%The best results are in bold.
}
\label{tab:stc_ave}

\resizebox{.8\columnwidth}{!}{%
\begin{tabular}{lcc}
% \cline{2-3}
\toprule
%  &  \textbf{HR STC} & \textbf{HR Avenue} \\ 

 &  \begin{tabular}[c]{@{}c@{}}\textbf{HR-STC}\end{tabular} & \textbf{HR-Avenue} \\ 
\midrule
Conv-AE \cite{hasan16}                                                                                                       & 69.8                                                             & 84.8      \\ %CONV-AE
Pred \cite{liu18}                                                                                                             & 72.7                                                            & 86.2      \\
MPED-RNN \cite{morais19}                                                                                                   & 75.4                                                            & 86.3      \\

GEPC \cite{markovitz20}                                                                                                        & 74.8                                                            & 58.1      \\

Normal Graph \cite{luo21}                                                                                          & 76.5                                                            & 87.3      \\

% \multicolumn{1}{c}{\citet{pang22}}                                                                                                      & \textbf{77.7}                                                            & 86.7      \\
COSKAD \cite{flaborea23}                                                                                                                  & 77.1                                                        & 87.3 \\ 
\midrule
\OUR                                                                                                                 & \textbf{77.5}                                                         & \textbf{88.0} \\

\bottomrule
\end{tabular}}
\vspace*{-4mm}


\end{table}
